NOELLE Offers Empowering LLVM Extensions

Modern and emerging architectures demand increasingly complex compiler analyses and transformations. As the emphasis on compiler infrastructure moves beyond support for peephole optimizations and the extraction of instruction-level parallelism, they should support custom tools designed to meet these demands with higher-level analysis-powered abstractions of wider program scope. This paper introduces NOELLE, a robust open-source domain-independent compilation layer built upon LLVM providing this support. NOELLE is modular and demand-driven, making it easy-to-extend and adaptable to custom-tool-specific needs without unduly wasting compile time and memory. This paper shows the power of NOELLE by presenting a diverse set of ten custom tools built upon it, with a 33.2% to 99.2% reduction in code size (LoC) compared to their counterparts without NOELLE.

==> Figs/llvm_invariant.tex <==
\begin{lstlisting}[morekeywords={}, aboveskip=0pt, belowskip=0pt, firstnumber=1]
bool isInvariant (
  Instruction I, Loop l,
  Dominator DT, AliasAnalysis AA){
  for (auto operand : I.getOperands()){
    if (operand is defined in L)  
      return false
  }

  if (isa<LoadInst>(I)){
    for (Instruction J : L){
      if (getModRef(J, I) != NoMod)
        return false
    }
  }

  if (isa<StoreInst>(I)){
    for (memory use MU in L){
      // Conservatively ensures no memory
      // use precedes this store
      if (!DT.dominates(I, MU))
        return false
    }
    // Ensures no memory def/use would be
    // invalidated by hoisting the store
    M=AA.getNearestDominatingMemoryAccess(I)
    if (M is in L) 
      return false
  }

  if (auto call = dyn_cast<CallInst>(I)){
    if (AA.getModRefBehavior(call) != NoMod)
      return false
    S=AA.onlyMemoryAccessesAreArguments(call)
    if (!S) 
      return false
    for (Argument A of call){
      for (auto subLoop : L->getSubLoops()){
        if (AA.getModRef(argument, anyLoopI)
            != NoMod) 
          return false
      }
    }
  }
  return true
}
\end{lstlisting}



==> Figs/noelle_invariant.tex <==
\begin{lstlisting}[morekeywords={}, aboveskip=0pt, belowskip=0pt, firstnumber=1]
bool isInvariant (
  Instruction I, Loop l,
  PDG dg, Stack s){
  if (I in s) 
    return false
  s.push(I)
  for (PDG dependency J -> I){
    if (J in L){
      inv = isInvariant(J, l, dg, s)
      if (!inv) 
        return false
    }
  }
  s.pop()
  return true
}

\end{lstlisting}


==> Sections/background.tex <==
NOELLE is the first open-source parallelizing compilation framework that
includes state-of-the-art parallelization techniques capable of parallelizing
irregular workloads. These techniques are
DSWP~\cite{1540952,Rangan:2008:PSD:1400112.1400113} and
HELIX~\cite{Campanoni:2012:HAP:2259016.2259028,6226338}. NOELLE also includes
DOALL~\cite{hurson1997parallelization} to parallelize loops with no
loop-carried data dependences better. This section provides information about
compiler concepts used throughout this paper and the aforementioned
parallelization techniques. Readers familiar with these concepts can skip to
Section~\ref{sec:solution}.

\subsection{Compiler Concepts}

% PDG
A \textbf{Program Dependence Graph} (PDG) is a graph where the nodes are the
instructions of a program and the edges represent either a data or a control
dependence~\cite{ferrante1987program}. Attributes are typically added to the
edges of a PDG to categorize dependences explicitly. Common attributes are the
type of dependence (i.e., Read-After-Write, Write-After-Write,
Write-After-Read), whether a dependence is via memory or variable (e.g.,
between a load and a store, between a variable definition and one of its use),
and whether it is a control or data dependence. For example, the PDG of the
code shown in Figure~\ref{fig:code_example_source} is shown in
Figure~\ref{fig:code_example_pdg}.

% SCC
\textbf{Strongly Connected Components} (SCC) are maximal strongly connected
subgraphs of a graph (the PDG in our case). For parallelizing compilers, SCCs
are related to a specific loop. For example, SCCs of the code shown in
Figure~\ref{fig:code_example_source} are highlighted in red in
Figure~\ref{fig:code_example_pdg}.

% SCCDAG
An \textbf{SCCDAG} is a directed acyclic graph generated from a PDG by
clustering instructions that belong to an SCC. For example,
Figure~\ref{fig:code_example_sccdag} is the SCCDAG of the PDG in
Figure~\ref{fig:code_example_pdg}. A node in an SCCDAG is either an instruction
or an SCC.

% Sequential segment
A \textbf{sequential segment} is a horizontal slice of a loop body that
includes an SCC~\cite{Campanoni:2012:HAP:2259016.2259028,6226338}. Hence, all
loop iterations must go through a sequential segment before jumping to the
subsequent one. For example, sequential segments of the code shown in
Figure~\ref{fig:code_example_source} are shown in
Figure~\ref{fig:code_example_ss}.

\begin{figure}[t]
\centering
\begin{minipage}{0.49\linewidth}
\subfloat[DSWP]
{
  \label{fig:code_example_DSWP}
  {\includegraphics[width=\textwidth]{Figs/eg_DSWP.pdf}}
}
\end{minipage}
\centering
\begin{minipage}{0.49\linewidth}
\subfloat[HELIX]
{
  \label{fig:code_example_HELIX}
  {\includegraphics[width=\textwidth]{Figs/eg_HELIX.pdf}}
}
\end{minipage}
\caption{
\label{fig:code_example_parallel}
DSWP and HELIX execution of Figure~\ref{fig:code_example}.
}
\end{figure}

\subsection{Parallelization Techniques}

This section describes the parallelization techniques included in NOELLE.

\paragraph{DSWP}
DSWP is a parallelization technique that extracts TLP from a loop by executing
its SCCs on different cores~\cite{1540952,Rangan:2008:PSD:1400112.1400113}. It
does so by enforcing a pipeline among the cores such that the communication
becomes acyclic. This approach makes DSWP insensitive to core-to-core
latencies. Figure~\ref{fig:code_example_DSWP} shows a DSWP execution of the
code shown in Figure~\ref{fig:code_example_source}.

%NOTE: The performance doesn't really scale this well.
%The TLP extracted by DSWP scales with the number of nodes that compose the SCCDAG of a loop.
Inter-core communication is mainly due to intra-loop iteration dependences
(i.e., to propagate values between SCCs).

\paragraph{HELIX}
HELIX is a parallelization technique that extracts TLP from a loop by executing
its iterations on different
cores~\cite{Campanoni:2012:HAP:2259016.2259028,6226338}. It does so by
exploiting the SMT characteristic of modern multicore processors to overlap
core-to-core communication with their computation. This overlap is performed by
one helper thread per physical core. Each helper thread runs ahead of time to
pre-start the communication that ends in its physical core.
Figure~\ref{fig:code_example_HELIX} shows a HELIX execution of the code shown
in Figure~\ref{fig:code_example_source}.

The TLP extracted by HELIX is limited by the core-to-core latency of the target
architecture. In other words, the faster the cores of an architecture can
communicate with each other, the more TLP can be extracted. Inter-core
communication is mainly due to loop-carried dependences (i.e., to propagate
values between instances of the same sequential segment).

\paragraph{DOALL}
DOALL is a parallelization technique that extracts TLP from a loop by executing
its iterations in parallel~\cite{hurson1997parallelization}. This technique can
be applied only if there is no loop-carried data dependence or if such a
dependency can be removed by transformations like
reduction~\cite{pottenger1995parallelization}.

The TLP extracted by DOALL is limited by the number of iterations of the target
loop. Inter-core communication is created to start and end the parallel
execution as well as to propagate live-in and live-out values with the code
outside the target loop. This communication is negligible compared to the one
performed by HELIX and DSWP. Hence, when DOALL is applicable, it is the
preferred parallelization technique as it provides the highest amount of TLP.
However, irregular workloads often have loops with non-removable loop-carried
data dependences. In those cases, DOALL is not applicable.


==> Tables/NOELLE.tex <==
\begin{table}[t]
\centering
\caption{
Source lines of code that compose NOELLE
}
\vspace{-1em}
\label{tab:NOELLE}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l|r|}
\hline
\textit{Module}       & \textit{LoC}  \\

\hline
\hline
PDG                        & 6775          \\
\hline                                 
aSCCDAG                    & 4517          \\
\hline                                 
Call graph                 & 620           \\
\hline                                 
Environment                & 991           \\
\hline                                 
Task                       & 297           \\
\hline 
Data-flow engine           & 332            \\
\hline 
Profiler                   & 1625           \\
\hline 
Scheduler                  & 1523           \\
\hline 
Loop builder               & 4535           \\
\hline 
Induction variables        & 352            \\
\hline 
Induction variable stepper & 425            \\
\hline
Loop                       & 1508           \\
\hline
Islands                    &   56           \\
\hline
Invariant                  &  137           \\
\hline 
Others                     & 2442           \\
\hline 
\textbf{LoC of NOELLE's abstractions} & \textbf{26142} \\

\hline                             
\hline                             
\texttt{noelle-whole-IR} & 1522  \\
\hline
\texttt{noelle-rm-lc-dependences}  & 912 \\
\hline                             
\texttt{noelle-prof-coverage} & 1761   \\
\hline         
\texttt{noelle-meta-prof-embed} & 152 \\
\hline
\texttt{noelle-meta-pdg-embed} & 451 \\
\hline
\texttt{noelle-load} & 12 \\
\hline
\texttt{noelle-arch} & 259    \\
\hline                             
\texttt{noelle-linker} & 59  \\
\hline
\texttt{noelle-bin} & 15  \\
\hline
\textbf{LoC of NOELLE's tools} & \textbf{5143} \\

\hline
\hline                             
Regression testing  & 5817 \\
\hline
Unit testing        & 2985 \\
\hline
Performance testing & 951  \\
\hline
\textbf{LoC of NOELLE's testing} & \textbf{9753} \\
\hline

\hline
\hline                             
\textbf{LoC of NOELLE } & \textbf{41038} \\
\hline

\end{tabular}
}
\end{table}

